Symmetric Arithmetic Circuits

We introduce symmetric arithmetic circuits, i.e. arithmetic circuits with a natural symmetry restriction. In the context of circuits computing polynomials defined on a matrix of variables, such as the determinant or the permanent, the restriction amounts to requiring that the shape of the circuit is invariant under simultaneous row and column permutations of the matrix. We establish unconditional exponential lower bounds on the size of any symmetric circuit for computing the permanent. In contrast, we show that there are polynomial-size symmetric circuits for computing the determinant over fields of characteristic zero.

==> sections-journal/equivariant.tex <==

Lower bounds for computing the permanent in symmetric models of computation have previously been established, notably in the work of Landsberg and Ressayre~\cite{LandsbergR16}.  They establish an exponential lower bound on the \emph{equivariant determinantal complexity} of the permanent, specifically over the complex field $\complex$.  In this section we make a brief comparison of our results with theirs.

The determinantal complexity (DC) of a polynomial $p \in \ff[X]$ is defined to be the least $m$ such that there is an $m\times m$ matrix $M$ with entries that are affine linear forms in $X$ such that $\det(M) = p$.  Such a matrix is called a \emph{determinantal representation} of $p$.  It is known~\cite{Valiant79} that every polynomial in $\VP$ has DC that is at most quasi-polynomial.  It follows that an exponential lower bound on the DC of the permanent would show that it is not in $\VP$, separating $\VP$ from $\VNP$.  Indeed, such a bound would 
show that circuits computing $\PERM_n$ must have size at least $2^{n^{\delta}}$ for some positive $\delta$.  On the other hand, an exponential lower bound on the circuit complexity of the permanent would also yield a similar lower bound for its determinental complexity.  To see this note that using an $O(n^3)$ family of circuits for computing $\{\DET_n\}$ and an $m\times m$ determinantal representation $M$ of the permanent, we get an $O(m^3)$ family of circuits computing $\{\PERM_n\}$.  This is obtained by taking the circuit computing the determinant and attaching to its $m^2$ inputs the circuits (of at most $O(n)$ size) computing the affine linear forms that form the entries of $M$.  Hence a $2^{f(n)}$ lower bound on the circuit complexity fo the permanent gives us a $2^{f(n)/3}$ upper bound on its determinantal complexity.

Landsberg and Ressayre establish exponential lower bounds on any \emph{equivariant} determinantal representation of the permanent, that is one that preserves all the symmetries of the permanent function.  This includes not just the
permutations on entries that we consider, but the entire projective symmetry
group.  Our aim is to see how this relates to our lower bounds on symmetric circuit complexity.  Unfortunately, the relationship is not straightforward in either direction because of the different notions of symmetry used and the symmetry-breaking nature of the translation from circuits to determinantal representations.  To make this explicit, we first introduce some definitions.  These are simplified from (and so less general than) those given by Landsberg and Ressayre but suffice to show that our results are incomparable with theirs. 

Formally, consider a homogeneous polynomial $p \in \complex[X]$.  Let $\GL_X$ denote the group of invertible linear maps on the vector space $\complex^X$.  
For a map $A \in \GL_X$, we write $p(AX)$ to mean the polynomial obtained from $p$ by replacing each variable $x \in X$ by the linear form $Ax$.  We now define the \emph{symmetry group} of $p$ to be the group $\mathcal{S}_p$ of linear maps $A \in \GL_X$ such that $p(AX) = p$.  In particular, when $X = \{x_{ij} \mid i,j \in [n] \}$ we can think of the elements of $\complex^X$ as $n \times n$ matrices and the symmetry group of $\DET_n$ can be identified with the group $\mathcal{S}_{\DET_n} = (\GL_n \times \GL_n)/\complex \times \ZZ_2$.  Here the action of $(A,B) \in  \GL_n \times \GL_n$ takes $V \in \complex^X$ to $AVB^{-1}/\det(AB^{-1})$ and the action of the non-trivial element in $\ZZ_2$ takes $V$ to $V^T$.

Let  $M$ be an $m\times m$ determinantal representation of a polynomial $p$.  For $A \in \GL_X$, write $M^A$ to be the matrix obtained from $M$ by replacing each entry $m$ by $Am$ (where we see each affine linear form $m$ as a polynomial in $\complex[X])$.   We say that $M$ is an \emph{equivariant} determinantal representation of $p$ if for each $A \in \mathcal{S}_p$ there is a $B \in \mathcal{S}_{\DET_n}$ such that $M^A = BM$.  In other words, all symmetries of $p$ extend to symmetries of $M$.    Landsberg and Ressayre prove that any equivariant determinantal representation of $\PERM_n$ must have size $\Omega(4^m)$.

We could ask if this lower bound yields a lower bound for symmetric circuits just as an exponential lower bound on the \emph{determinantal complexity} of the permanent yields a lower bound for its unrestricted circuit complexity.  This would require a translation, along the lines of Valiant~\cite{Valiant79} from symmetric circuits to equivariant determinantal representations.  There is little reason to believe that we could have such a translation.  For one thing, the symmetry requirement for \emph{square-symmetric} circuits is only that they are invariant under the natural action of $\sym_n$ on $\PERM_n$, and this is a rather small subgroup of $\mathcal{S}_{\PERM_n}$.  Secondly, Valiant's translation of circuits to determinantal representations is not symmetry preserving.  Thus, the representations obtained from this translation applied to square-symmetric circuits are not even guaranteed to be equivariant with respect to the action of $\sym_n$ on $\PERM_n$, let alone that of $\mathcal{S}_{\PERM_n}$.

In the other direction, we could ask if our lower bounds for symmetric circuits for the permanent yield any lower bounds for equivariant determinantal complexity, especially in combination with the polynomial upper bound for transpose-symmetric circuits for the determinant proved in Theorem~\ref{thm:det-upper-bound}.  Indeed, given a circuit $C$ of size $s$ computing $\DET_m$ and an $m\times m$ determinantal representation $M$ of $p$, a polynomial on $n$ variables, we obtain a circuit $C'$ computing $p$ of size $s(m)+ O(nm)$, where the second term represents the size of the subcircuits required to compute the affine expressions making up the entries of $M$.  If an equivariant determinantal expression translates to a symmetric circuit, then a symmetric circuit lower bound can be translated to a lower bound on equivariant determinantal complexity.  Since the symmetry conditions for circuits are less restrictive, this seems plausible, but there is a mismatch.

Consider the case when $p$ is $\PERM_n$, and $C$ is the square-symmetric circuit for $\DET_m$ obtained from Theorem~\ref{thm:det-upper-bound}.  For the circuit $C'$ to be square symmetric, we require that the action of $\sym_n$ on the variables $X =\{x_{ij} \mid i,j \in [n]\}$ extends to automorphisms of the circuit.  Since this action gives a subgroup of $\mathcal{S}_{\PERM_n}$ acting on $\PERM_n$, we know that for each $\pi \in \sym_n$ there is a $B \in \mathcal{S}_{\DET_m}$ such that $M^{\pi} = BM$.  If this map $B$ was itself the action of a permutation in $\sym_m$ on the rows and columns of $M$, the square symmetry of $C$ would guarantee that $C'$ was also square-symmetric.  However, the equivariance of $M$ does not enforce this.  So, to state the lower bound on determinantal complexity that we can get from our results, we define an alternative notion of equivariance.

Say that $M$ is \emph{permutation equivariant} if for each $\pi \in \sym_n$, there is a permutation matrix $B \in \GL_m$ such that $M^{\pi} = BM$.  Note that this notion is incomparable with equivariance of $M$.  We have relaxed the requirement by only asking that permutation matrices in $\mathcal{S}_{\PERM_n}$ extend to symmetries of $M$, but we have made it more stringent by asking that the symmetry they extend to is itself a permutation matrix in $\mathcal{S}_{\DET_m}$.  We can now state the following corollary of our results.
\begin{corollary}
Any permutation equivariant determinantal representation of $\PERM_n$ has size $2^{\Omega(n)}$.
\end{corollary}




